On the cohomology of simple Shimura varieties with non quasi-split local groups

We study the Scholze test functions for bad reduction of simple Shimura varieties at a prime where the underlying local group is any inner form of a product of Weil restrictions of general linear groups. Using global methods, we prove that these test functions satisfy a vanishing property of their twisted orbital integrals, and we prove that the pseudostabilization base changes of such functions exist (even though the local group need not be quasi-split) and can be expressed in terms of explicit distributions in the stable Bernstein center. We then deduce applications to the stable trace formula and local Hasse-Weil zeta functions for these Shimura varieties.

==> matching.tex <==
{\cp
It is well-known that to check the matching of (twisted) orbital integrals on all semisimple elements it suffices to check the matching on \emph{regular} semisimple elements. For the reader's convenience we include a proof of this fact in our setting, following the arguments of \cite[Prop.\,7.2]{Clo90}.}
{\cp 
\begin{prop} We have the following two statements.
\begin{enumerate}
\item[(1)] Let $\phi\in C_c^\infty(G_r)$ and $\phi^*\in C_c^\infty(G^*)$. Suppose that for any \emph{regular} $\bbQ_p$-elliptic semisimple element $\ga^*\in G^*$ we have $O_{\ga^*}(\phi^*)=0$ if $\ga^*$ is not a norm from $G_r$, while if $\ga^*=\cN_r\delta$ we have
    \[O_{\ga^*}(\phi^*)=TO_{\delta\sigma}(\phi).\]
    Then $\phi^*$ is a stable base change transfer of $\phi$ at all $\bbQ_p$-elliptic semisimple elements $\ga^*$.
    \item[(2)] If $\phi$ satisfies the vanishing property, then the above statement holds without the qualifier ``elliptic''.
\end{enumerate}    
\end{prop}
}
\begin{proof} 
{\cp Suppose $\ga^*=\cN_r\delta$ is an semisimple element in $G^*$. By \cite[Lem.\,5.8]{Ko-conj}, once we fix an $\bbQ_p$-inner twisting $\bfG \rightarrow \bfG^*$ there is an $\bbQ_p$-inner twisting $\bfG_{\delta \sigma} \rightarrow \bfG^*_{\ga^*}$, canonical up to inner automorphisms by $\bfG^*_{\ga^*}(\bar{\bbQ}_p)$. For any maximal $\bbQ_p$-torus ${\mathbf T} \subset \bfG_{\delta\sigma}$ (at the moment ${\mathbf T}$ need not be $\bbQ_p$-elliptic), we may assume our inner twisting induces a $\bbQ_p$-embedding ${\mathbf T} \hookrightarrow \bfG^*_{\ga^*} \subset \bfG^*$, by \cite[Cor.\,2.2]{Ko-conj}. Fix a Haar measure $dt$ on $T := {\mathbf T}(\bbQ
_p)$. Let $\{u_j\}$ be a set of representatives of unipotent conjugacy classes in $G_{\delta\sigma}$. It follows from \cite[Proposition 8.1.1]{Ro90} that there is a sufficiently small neighborhood $0\in\Omega\subset\mathrm{Lie}(T)$ such that 
\begin{itemize}
    \item the exponential map defines an isomorphism from $\Omega$ to an open neighborhood of $1$ in $T$;
    \item Let $\Omega'\subset\Omega$ be the open subset consisting of elements $X\in\Omega$ such that $\exp(X)\in T$ is regular. Then $a\Omega'\subset\Omega'$ for any $0\ne a\in\bbZ_p$;
    \item The germ expansion holds on $\Omega'$, i.e.\,for all $0\ne t\in\bbZ_p$ and any $X\in\Omega'$, denote $x_t:=\exp(tX)$, then we have
    \[TO_{x_t\delta\sigma}(\phi)=\sum_j\Gamma_{u_j}^G(x_t\delta)\,TO_{u_j\delta\sigma}(\phi),\quad\forall \phi\in C_c^\infty(G_r)\]
    where the Shalika germ $\Gamma_{u_j}$ is a function on $\exp(\Omega')\delta$ that depends on the Haar measure on $T=G_{x_t\delta\sigma}=(G_{\delta\sigma})_{x_t}$ and the Haar measure on $G_{u_j\delta\sigma}$ used to define the orbital integrals. 
\end{itemize}
By \cite[Proposition 8.1.2(b)]{Ro90}, the function $\Gamma_{u_j}^G$ is homogeneous of degree $\frac{1}{2}d_{u_j}:=\frac{1}{2}\dim(G_{\delta\sigma}/G_{u_j\delta\sigma})$ in the sense that for all $X\in\Omega'$ and $0\ne t\in\bbZ_p$ we have
\[\Gamma_{u_j}^G(\exp(tX)\delta)=|t|^{-\frac{1}{2}d_{u_j}}\Gamma_{u_j}^G((\exp X)\delta).\]
By \cite[Proposition 8.1.2(a)]{Ro90} we have 
\[\Gamma_{1}^G((\exp X)\delta)=\Gamma_{1}^{G_{\delta\sigma}}(\exp X).\]
{\cb At this point we assume that $\ga^*$ is $\bbQ_p$-elliptic and is contained in an elliptic maximal torus ${\mathbf T}^* \subset \bfG^*$; then we can arrange that ${\mathbf T}$ is also elliptic and our chosen inner twisting $\psi$ gives a $\bbQ_p$-isomorphism $\psi: {\mathbf T} \overset{\sim}{\rightarrow} {\mathbf T}^*$. Then we have $N_r\delta \in T$ and $\psi(N_r\delta) = \ga^*$. Now the main theorem of \cite{Ro80} shows that}
\[\Gamma_{1}^{G_{\delta\sigma}}(\exp X)=(-1)^{q(G_{\delta\sigma})}d(G_{\delta\sigma})^{-1},\quad\forall X\in\Omega'\] 
where $q(G_{\delta\sigma})$ is the $\bbQ_p$-rank of the derived group of $G_{\delta\sigma}$ and $d(G_{\delta\sigma})$ is the formal degree of the Steinberg representation of $G_{\delta\sigma}$ (with respect to a chosen Haar measure on $G_{\delta\sigma}$). Consequently we have
\[TO_{x_t\delta\sigma}(\phi)=(-1)^{q(G_{\delta\sigma})}d(G_{\delta\sigma})^{-1}TO_{\delta\sigma}(\phi)+A(t),\quad\forall0\ne t\in\bbZ_p\]
where $A(t)$ is a linear combination of functions $|t|^{-a}$ with $a>0$. \par 
For untwisted orbital integrals we have a similar result which is proved in \cite[\S3]{Ko-Tam} in complete generality. In our setting, if $\ga^*=\cN_r\delta\in G^*$ is the norm of $\delta$, then we have 
    \[O_{\psi(x_t)\ga^*}(\phi^*)=(-1)^{q(G^*_{\ga^*})}d(G^*_{\ga^*})^{-1}O_{\ga^*}(\phi^*)+B(t)\]
where $B(t)$ is a linear combination of functions $|t|^{-a}$ with $a>0$. In \cite{Ko-Tam}, the measure on the groups are determined from Euler-Poincar\'e measures on adjoint groups, in which case $d(G^*_{\ga^*})=(-1)^{q(G^*_{\ga^*})}$ by \cite{Bo76} (see also \cite[\S7.1]{GR}). Then by \cite[Theorem 1]{Ko-Tam}, if the measures on $G_{\delta\sigma}$ and $G^*_{\ga^*}$ are chosen compatibly, we have $d(G_{\delta\sigma})=d(G^*_{\ga^*})$. From the definition we verify easily that for any $X\in\Omega'$ and $0\ne t\in\bbZ_p$ we have $N_r(\exp(tX)\delta)=\exp(rtX)N_r\delta$ and hence under our chosen embedding $T\into G^*_{\ga^*}$ we have $\cN_r(\exp(tX)\delta)=\psi(\exp(rtX))\ga^*$. This also shows that if $\ga^*$ is not conjugate to a norm from $G_r$, then $\psi(\exp(rtX))\ga^*$ is also not conjugate to a norm from $G_r$. Then from the assumption we have 
\[TO_{\exp(tX)\delta\sigma}(\phi)=O_{\exp(rtX)\ga^*}(\phi^*)\]
if $\ga^*=\cN_r\delta$ and $O_{\exp(rtX)\ga^*}(\phi^*)=0$ if $\ga^*$ is not a norm from $G_r$. Comparing the degree $0$ part of both sides we get
\[TO_{\delta\sigma}(\phi)=(-1)^{q(G_{\delta\sigma})-q(G^*_{\ga^*})}O_{\ga^*}(\phi^*)\]
if $\ga^*=\cN_r\delta$ and $O_{\ga^*}(\phi^*)=0$ if $\ga^*$ is not a norm from $G_r$.\par 

Finally we note that since $G^*_{\ga^*}$ is the quasi-split inner form of $G_{\delta\sigma}$, we have $e(G^*_{\ga^*})=1$ and $e(G_{\delta\sigma})=(-1)^{q(G_{\delta\sigma})-q(G^*_{\ga^*})}$.}
{\cb The above completes the proof of (1), that is, for the case where $\ga^*$ is $\bbQ_p$-elliptic in $G^*$.  By the lemma below, if $\phi$ satisfies the vanishing property, we can reduce to this case by a descent argument, and this will complete the proof of (2).}
\end{proof}

We now discuss the descent argument. We assume $\ga^* in G^*$ is semisimple. If $\ga^*$ is $\bbQ_p$-elliptic in $G^*$, the above proof of (1) suffices. If not, then there is a $\bbQ_p$-Levi subgroup ${\mathbb M}^* \subset \bfG^*$ containing $\ga^*$ such that ${\mathbf M}^*_{\ga^*} = \bfG^*_{\ga^*}$, and $\ga^*$ is $\bbQ_p$-elliptic in $M^*$.  

If $\ga^*$ is not a norm from $G_r$, we must show that $O_{\ga^*}(\phi^*) = 0$.  Using the above argument, noting that none of the elements $\exp(rtX)) \ga^*$ are norms from $G_r$, this follows by the vanishing of the degree $0$ part of the Shalika germ expansion
    \[O_{\exp(rtX)\ga^*}(\phi^*)=\sum_j\Gamma_{u_j}^{G^*}(\exp{rtX}\ga^*)\,O_{u_j\ga^*}(\phi^*),\quad\forall t \in \mathbb Z_p, \,t\neq 0.\]

Now suppose $\ga^*$ is a norm from $G_r$.  There are two subcases: ${\mathbf M}^*$ transfers to ${\bf G}$, or it does not transfer.  





{\cg Tom: I don't have a complete proof of the descent lemma.  We assume $\ga^* \in M^*$ with $M^*_{\ga^*} = G^*_{\ga^*}$ and $\ga^*$ elliptic in $M^*$.  If $M^*$ is the transfer from $G$ of a Levi $M$ in $G$, then we may prove that $\ga^*$ being a norm from $G_r$ implies it is a norm from $M_r$, and then the formulas for descent of orbital integrals give the result.  However, I don't know what to do when $M^*$ is not a transfer of a Levi from $G$.  We have to rule this out somehow.  By the way, is this proposition needed in full force, or is only the elliptic case of the proposition needed? We would LIKE a result like the following.}

{\cg
\begin{lem}
Suppose $\ga^* \in G^*$ is semisimple and there is a $\bbQ_p$-Levi subgroup ${\mathbf M}^* \subset \bfG^*$ such that ${\mathbf M}^*_{\ga^*} = \bfG^*_{\ga^*}$ and $\ga^*$ is $\bbQ_p$-elliptic in ${\mathbf M}^*$. Suppose that $\ga^* = \mathcal N_r\delta$ for some $\delta \in G_r$  Then 
\begin{enumerate}
\item[(a)] ${\mathbf M}^*$ transfers to a $\bbQ_p$-Levi ${\mathbf M}$ of $\bf G$;
\item[(b)] $\delta$ is $G_r$-$\sigma$-conjugate to an element $\delta_1 \in M_r$, such that $\mathcal N_r\delta_1 = \ga^*$ in $M^*$.
\end{enumerate}
\end{lem}

\begin{proof}
By Kottwitz [REF], there is a $\bbQ_p$-inner twisting $\psi: \bfG^*_{\ga^*} \rightarrow \bfG_{\delta \sigma}$. Choose an elliptic torus ${\mathbf T}^* \subset {\mathbf M}^*$ containing $\ga^*$.  By Kottwitz [REF] it transfers to $\bfG_{\delta\sigma}$, and we may assume $\psi({\mathbf T}^*) = {\mathbf T}$, a maximal $\bbQ_p$-torus in $\bfG_r$.  Let $A_{M^*}$ be the connected center of ${\mathbf M}^*$, and identity it via $\psi$ with a subtorus $A_{M^*} \subset \bfG_r$. The morphism $A_{M^*} \rightarrow \bfG_r$ corresponds to an embedding $A_{M^*,\bbQ_{p^r}} \rightarrow \bfG_{\bbQ_{p^r}}$, which factors through $A_{0} \subset \bfG_{\bbQ_{p^r}}$,....unfortunately one cannot get any further, and in general it is NOT automatic that ${\mathbf M}^*$ transfer to $G$.  The hope would be that IF $O_{\ga^*}( f_{M^*}) \neq 0$, and $f$ is a transfer of $\phi_r$, then in this case ${\bf M}^*$ must transfer. This is ok in the untwisted case...
\end{proof}
}

{\cg Tom: UPDATE of 06/23/2024: I think we might be able to prove the following: if $(\phi, \phi^*)$ as above, and we assume in addition that $\phi$ satisfies the vanishing property, then the matching at all regular semisimple $\ga^*$ implies the matching at all semisimple $\ga^*$. The point should be: if $M^*$ does not transfer, then we get both sides vanish for all regular $\ga^*$ in $M^*$ and all $\delta$ matching with $\ga^*$, since none of those $\delta$ are rational (if they were, then the regular $\ga^*$ would transfer to rational elements in $G$, and then the maximal torus $T^* \subset M^*$ would transfer, and then $A_{M^*}$ would transfer, and then $M^*$ itself would transfer.  On the other hand, if $M^*$ does transfer, then the descent formulas give the result once we cite the lem above.}


